Stochastic Training of Graph Convolutional Networks with Variance Reduction

Graph convolutional networks (GCNs) are powerful deep neural networks for graph-structured data. However, GCN computes the representation of a node recursively from its neighbors, making the receptive field size grow exponentially with the number of layers. Previous attempts on reducing the receptive field size by subsampling neighbors do not have a convergence guarantee, and their receptive field size per node is still in the order of hundreds. In this paper, we develop control variate based algorithms which allow sampling an arbitrarily small neighbor size. Furthermore, we prove new theoretical guarantee for our algorithms to converge to a local optimum of GCN. Empirical results show that our algorithms enjoy a similar convergence with the exact algorithm using only two neighbors per node. The runtime of our algorithms on a large Reddit dataset is only one seventh of previous neighbor sampling algorithms.

==> 91-thm1.tex <==
\section{Proof of Theorem 1}\label{sec:proof-of-thm1}
\begin{reptheorem}{M-thm:prediction}
	\exacttesting
\end{reptheorem}

\begin{proof}
We prove by induction.  After the first epoch the activation $h^{(0)}_{i,v}$ is at least computed once for each node $v$. 
So $\bar H_{CV, i}^{(0)}=H_{CV, i}^{(0)}=H^{(0)}=X$ for all $i>I$. 
%
Assume that we have $\bar H_{CV, i}^{(l)}=H_{CV, i}^{(l)}=H^{(l)}$ for all $i>(l+1)I$. 
Then for all $i>(l+1)I$
\begin{align}
Z_{CV, i}^{(l+1)}&=\left(\hat P^{(l)}_i (H_{CV, i}^{(l)}-\bar H_{CV, i}^{(l)}) + P\bar H_{CV, i}^{(l)}\right) W^{(l)} = P\bar H_{CV, i}^{(l)}W^{(l)} = P  H^{(l)} W^{(l)} = Z^{(l+1)}.\label{eqn:thm1-rec}\\
H_{CV, i}^{(l+1)}&=\sigma(Z_{CV,i}^{(l+1)})=H^{(l+1)}\nonumber 
\end{align}
After one more epoch, all the activations $h_{CV, i, v}^{(l+1)}$ are computed at least once for each $v$, so $\bar H_{CV, i}^{(l+1)}=H_{CV, i}^{(l+1)}=H^{(l+1)}$ for all $i>(l+2)I$. 
By induction, we know that after $LI$ steps, we have
$\bar H_{CV, i}^{(L-1)} = H_{CV, i}^{(L-1)} = H^{(L-1)}$. By Eq.~\ref{eqn:thm1-rec} we also have $\bar Z_{CV, i}^{(L)} = Z^{(L)}$. 

\end{proof}





















==> 92-thm2.tex <==
% !TeX spellcheck = en_US
\section{Proof of Theorem 2}\label{sec:proof-of-thm2}
We proof Theorem~\ref{M-thm:convergence} in 3 steps:
\begin{enumerate}
\item Lemma~\ref{proposition2}: For a sequence of weights $W^{(1)}, \dots, W^{(N)}$ which are close to each other, CV's approximate activations are close to the exact activations.
\item Lemma~\ref{gradient-bound-lemma}: For a sequence of weights $W^{(1)}, \dots, W^{(N)}$ which are close to each other, CV's gradients are close to be unbiased.
\item Theorem~\ref{M-thm:convergence}: An SGD algorithm generates the weights that changes slow enough for the gradient bias goes to zero, so the algorithm converges. 
\end{enumerate}

The following proposition is needed in our proof
\begin{proposition}
Let $\inorm{A}=\max_{ij}\abs{A_{ij}}$, then
\begin{itemize}
    \item $\inorm{AB} \le col(A) \inorm{A}\inorm{B}$, where $col(A)$ is the number of columns of the matrix $A$.
    \item $\inorm{A\circ B}\le \inorm{A}\inorm{B}$, where $\circ$ is the element wise product.
    \item $\inorm{A+B}\le \inorm{A}+\inorm{B}$.
\end{itemize}
\end{proposition}
\begin{proof}
\begin{align*}
	\inorm{AB} &= \max_{ij}\abs{\sum_k A_{ik} B_{ik}} \le \max_{ij}\abs{\sum_k \inorm{A}\inorm{B}} = col(A) \inorm{A}\inorm{B}.\\
	\inorm{A\circ B}&= \max_{ij} \abs{A_{ij} B_{ij}} \le \max_{ij} \inorm{A} \inorm{B} = \inorm{A}\inorm{B}.\\
	\inorm{A+B}&=\max_{ij}\abs{A_{ij}+B_{ij}}\le
	\max_{ij}\left\{\abs{A_{ij}}+\abs{B_{ij}}\right\}\le
	\max_{ij}\abs{A_{ij}} + \max_{ij}\abs{B_{ij}}
	=\inorm{A}+\inorm{B}.
\end{align*}
\end{proof}
We define $C:=\max\{col(P), col(H^{(0)}), \dots, col(H^{(L)})\}$ to be the maximum number of columns we can possibly encounter in the proof.






\subsection{Single layer GCN}
The following proposition states that if the inputs and the weights of an one-layer GCN with CV estimator does not change too much, then its output does not change too much, and is close to the output of an exact one-layer GCN.
\begin{proposition}
If the activation $\sigma(\cdot)$ is $\rho$-Lipschitz, 
for any series of $T$ inputs, weights, and stochastic propagation matrices $(X_i, X_{CV, i}, W_i, \hat P_i)_{i=1}^T$, s.t., 
\begin{enumerate}
	\item all the matrices are bound by $B$, i.e., $\inorm{X_{CV, i}}\le B$, $\inorm{X_i}\le B$, $\inorm{W_i}\le B$ and $\inorm{\hat P_i}\le B$,
	\item the differences are bound by $\epsilon$, i.e., 
	$\inorm{X_{CV, i}-X_{CV, j}}<\epsilon$, $\inorm{X_{CV, i}-X_{i}}<\epsilon$ and $\inorm{W_i-W_j}<\epsilon$,
\end{enumerate}
let $P=\E \hat P_i$. 
If at time $i$ we feed $(X_{CV, i}, W_i, \hat P_i)$ to an one-layer GCN with CV estimator to evaluate the prediction for nodes in the minibatch $\Vc_i$, \footnote{Conceptually we feed the data for all the nodes in $\Vc$, but since we only require the predictions for the nodes in $\Vc_i$, the algorithm will only fetch the input of a subset of nodes $\subset \Vc$, and update history for those nodes.}
$$Z_{CV, i}=\left(\hat P_i(X_{CV, i} - \bar X_{CV, i}) + P\bar X_{CV, i}\right) W_i, \quad H_{CV, i}=\sigma(Z_{CV, i}).$$
where $\bar X_{CV, i}$ is the maintained history at time $i$, and $(X_{i}, W_i, P)$ to an one-layer GCN with exact estimator
$$Z_i=P X_i W_i, \quad H_i=\sigma(Z_i),$$
then there exists $K$ that depends on $C$, $B$ and $\rho$, s.t. for all $I<i, j\le T$, where $I$ is the number of iterations per epoch:
\begin{enumerate}
	\item The outputs does not change too fast: $\inorm{Z_{CV, i}-Z_{CV, j}}<K\epsilon$ and $\inorm{H_{CV, i}-H_{CV, j}}<K\epsilon$,
	\item The outputs are close to the exact output: $\inorm{Z_{CV, i}-Z_{i}}<K\epsilon$ and $\inorm{H_{CV, i}-H_{i}}<K\epsilon$.
\end{enumerate}
\end{proposition}\label{proposition1}
\begin{proof}
Because for all $i>I$ (i.e., after one epoch), the elements of $\bar X_{CV, i}$ are all taken from previous iterations, i.e., $X_{CV, 1}, \dots, X_{CV, i-1}$, we know that 
\begin{align}
\inorm{\bar X_{CV, i} - X_{CV, i}} \le \max_{j\le i} \inorm{X_{CV, j} - X_{CV, i}} \le \epsilon\quad (\forall i>I).
\end{align}
By triangular inequality, we also know
\begin{align}
\inorm{\bar X_{CV, i} - \bar X_{CV, j}} &< 3\epsilon \quad (\forall i, j>I).\\
\inorm{\bar X_{CV, i} - X_{i}} &< 2\epsilon \quad (\forall i>I).
\end{align}
Since $\inorm{X_{CV, 1}}, \dots, \inorm{X_{CV, T}}$ are bounded by $B$, $\inorm{\bar X_{CV, i}}$ is also bounded by $B$ for $i>I$. Then,
\begin{align*}
&\inorm{Z_{CV, i}-Z_{CV, j}} \\
=& \inorm{\left(\hat P_i(X_{CV, i} - \bar X_{CV, i}) + P\bar X_{CV, i}\right) W_i - \left(\hat P_j(X_{CV, j} - \bar X_{CV, j}) + P\bar X_{CV, j}\right) W_j}\\
\le& \inorm{\hat P_i(X_{CV, i} - \bar X_{CV, i})W_i - \hat P_j (X_{CV, j} - \bar X_{CV, j})W_j} + \rho \inorm{P\bar X_{CV, i} W_i - P\bar X_{CV, j} W_j} \\
\le& C^2[ 
\inorm{\hat P_i-\hat P_j}\inorm{X_{CV, i} - \bar X_{CV, i}} \inorm{W_i}\\
&+\inorm{\hat P_j}   \inorm{X_{CV, i} - \bar X_{CV, i} - X_{CV, j} + \bar X_{CV, j}}      \inorm{W_i}\\
&+\inorm{\hat P_j} \inorm{X_{CV, j}-\bar X_{CV, j}} \inorm{W_i-W_j}\\
&+\inorm{P}\inorm{\bar X_{CV, i}-\bar X_{CV, j}}\inorm{W_i}\\
&+\inorm{P}\inorm{\bar X_{CV, j}}\inorm{W_i-W_j}
]\\
\le& C^2\epsilon[
\inorm{\hat P_i-\hat P_j}\inorm{W_i} + 
2\inorm{\hat P_j}\inorm{W_i} + 
\inorm{\hat P_j}\inorm{W_i-W_j} \\
+&3\inorm{\hat P_j}\inorm{W_i} + \inorm{\hat P_j}\inorm{\bar X_{CV, j}}
]\\
\le& \epsilon C^2\left[2B^2+2B^2+2B^2+3B^2+B^2\right]\\
=&K_1\epsilon,
\end{align*}
where $K_1=10 C^2 B^2$,
and 
\begin{align*}
\inorm{Z_{CV, i}-Z_i} 
&\le \inorm{\left(\hat P_i(X_{CV, i} - \bar X_{CV, i}) + P(\bar X_{CV, i} - X_i)\right)} \inorm{W_i}  \\
&\le  C (\inorm{\hat P_i}\epsilon + 2\inorm{P}\epsilon)\inorm{W_i}\\
&\le  3 CB^2 \epsilon \\
&= K_2\epsilon,
\end{align*}
where $K_2 = 3 CB^2$. By Lipschitz continuity
\begin{align*}
\inorm{H_{CV, i}-H_{CV, j}}  &\le \rho K_1 \epsilon,\\
\inorm{H_{CV, i}-H_i}        &\le \rho K_2 \epsilon.\\
\end{align*}
We just let $K=\max\{\rho K_1, \rho K_2, K_1, K_2\}$.
\end{proof}



\subsection{Lemma~\ref{proposition2}: Activation of Multi-layer GCN}
The following lemma bounds the approximation error of activations in a multi-layer GCN with CV. Intuitively, there is a sequence of slow-changing model parameters $(W_i)$, where $W_i$ is the model at the $i$-th iteration. At each iteration $i$ we use GCN with CV and GCN with Exact estimator to compute the activations for the minibatch $\Vc_i$, and update the corresponding history. Then after $L$ epochs, the error of the predictions by the CV estimator is bounded by the rate of change of $(W_i)$, regardless of the stochastic propagation matrix $\hat P_i$.

\begin{lemma}\label{proposition2}
Assume all the activations are $\rho$-Lipschitz, given a fixed dataset $X$ and a sequence of $T$ model weights and stochastic propagation matrices $(W_i, \hat P_i)_{i=1}^T$, s.t.,
\begin{enumerate}
	\item $\inorm{W_i}\le B$ and $\inorm{\hat P_i}\le B$,
	\item $\inorm{W_i-W_j}<\epsilon, \forall i, j$,	
\end{enumerate}
let $P=\E \hat P_i$. 
If at time $i$ we feed $(X, W_i, \hat P_i)$ to a GCN with CV estimator to evaluate the prediction for nodes in the minibatch $\Vc_i$,
$$Z_{CV, i}^\bll=\left(\hat P_i^\bl(H_{CV, i}^\bl - \bar H_{CV, i}^\bl) + P\bar H_{CV, i}^\bl\right) W_i^\bl, \quad H_{CV, i}^\bll=\sigma(Z_{CV, i}^\bll).$$
where $\bar H_{CV, i}^\bl$ is the maintained history at time $i$, and $(X, W_i, P)$ to a GCN with exact estimator
$$Z_i^\bll=P H_i^\bl W_i^\bl, \quad H_i^\bll=\sigma(Z_i^\bll),$$
then there exists $K$ that depends on $C$, $B$ and $\rho$
 s.t., 
\begin{itemize}
\item $\inorm{H_i^{\bL}-H_{CV, i}^\bL}<K\epsilon, \forall i>LI, l=1, \dots, L-1$,
\item $\inorm{Z_i^{\bL}-Z_{CV, i}^\bL}<K\epsilon, \forall i>LI, l=1, \dots, L$.
\end{itemize}
\end{lemma}
\begin{proof}
By Proposition~\ref{proposition1}, we know there exists $K^{(1)}$, s.t., 
$\norm{H_i^{(1)} - H_{CV, i}^{(1)}} < K^{(1)}\epsilon$ and $\norm{H_{CV, i}^{(1)} - H_{CV, j}^{(1)}} < K^{(1)}\epsilon$, $\forall i>I$. 

Repeat this for $L-1$ times, we know there exist $K^{(1)}, \dots, K^{(L)}$, s.t., 
$\norm{H_i^{(L)} - H_{CV, i}^{(L)}} < K\epsilon$, $\norm{H_{CV, i}^{(L)} - H_{CV, j}^{(K)}} < K\epsilon$, 
$\norm{Z_i^{(L)} - Z_{CV, i}^{(L)}} < K\epsilon$ and $\norm{Z_{CV, i}^{(L)} - Z_{CV, j}^{(K)}} < K\epsilon$, 
$\forall i>LI$, where $K=\prod_{l=1}^L K^{(l)}$.



%Because $H^{(0)}=X$ is constant, $\bar H_{CV, i}^{(0)}=H_i^{(0)}$ after $I$ iterations. So $H^{(1)}_{CV, i}=\sigma(\left(\hat P_i(H^{(0)}_{CV, i}-\bar H^{(0)}_{CV, i})+P\bar H^{(0)}_{CV, i}\right)W^{(0)}_i=\sigma(PXW^{(0)}_i)=H^{(1)}_i$, and 
%\begin{align*}
%\inorm{H^{(1)}_{CV, i}-H^{(1)}_{CV, j}} = \inorm{ \sigma(PXW^{(0)}_i)-\sigma(PXW^{(0)}_j) } \le \rho C \inorm{P} \inorm{X} \epsilon_0. 
%\end{align*}
%Repeatedly apply Proposition~\ref{proposition1} for $L-1$ times, we get the intended results.
\end{proof}







\subsection{Lemma~\ref{gradient-bound-lemma}: Gradient of Multi-layer GCN}
We reiterate some notations defined in Sec.~\ref{M-sec:theory} of the main text. $\Vc_i$ is the minibatch of nodes at iteration $i$ that we would like to evaluate the predictions and gradients on.  
$g_{CV,v}(W_i):=\nabla f(y_v, z_{CV,i,v}^\bL)$ is the stochastic gradient propagated through the node $v$ by the CV estimator, and 
$g_{CV,i}(W_i):=\frac{1}{|\Vc_i|}\sum_{v\in \Vc_i} \nabla f(y_v, z_{CV,i,v}^\bL)$ is the minibatch gradient by CV. 
$g_{v}(W_i):=\nabla f(y_v, z_{v}^\bL)$ is stochastic gradient propagated through the node $v$ by the Exact estimator, and $g_{i}(W_i):=\frac{1}{|\Vc_i|}\sum_{v\in \Vc_i} \nabla f(y_v, z_{v}^\bL)$ is the minibatch gradient by the Exact estimator. Finally, $\nabla \Lc(W_i)=\frac{1}{|\Vc_{\Lc}|}\sum_{v\in \Vc_{\Lc}} \nabla f(y_v, z_{i,v}^\bL)$ is the exact full-batch gradient.

The following lemma bounds the bias of the gradients by the CV estimator. Intuitively, there is a sequence of slow-changing model parameters $(W_i)$, where $W_i$ is the model at the $i$-th iteration. At each iteration $i$ we use GCN with CV and GCN with Exact estimator to compute the activations for the minibatch $\Vc_i$, and update the corresponding history. After $L$ epochs, we compute the gradient by backpropagating through CV's predictions on the minibatch of nodes $\Vc_i$. 
The gradient $g_{CV,i}(W_i)$ is a random variable of both the stochastic propagation matrix $\hat P_i$ and the minibatch $\Vc_i$. But the expectation of the gradient w.r.t. $\hat P_i$ and $\Vc_i$, $\E_{\hat P_i, \Vc_i} g_{CV, i}(W_i)$, is close to the full-batch gradient by the Exact estimator $\nabla \Lc(W_i)$, i.e., the gradient is close to be unbiased. 


To study the gradient, we need the backpropagation rules of the networks. Let $f_v=f(y_v, z^\bL_v)$ and $f_{CV,i,v}=f(y_z, z^\bL_{CV,i,v})$, we first derive the backpropagation rule for the exact algorithm. 
Differentiating both sides of Eq.~(\ref{M-eqn:gcn}), we have:
\begin{align}
	\nabla_{\HL} \loss &= P^{\top} \nabla_{\ZLp} \loss \WLT                 & l=1, \dots, L-1 \nonumber \\
	\nabla_{\ZL} \loss &= \sigma^\prime(\ZL) \circ \nabla_{\HL} \loss       &   l=1, \dots, L-1 \nonumber \\
	\nabla_{\WL} \loss &= (P \HL)^\top \nabla_{\ZLp} \loss                  & l=0, \dots, L-1.\label{eqn:gcn-backprop} 
\end{align}
Similarly, differentiating both sides of Eq.~(\ref{M-eqn:cv}), we have
\begin{align}
\nabla_{\HLcv} \cvloss &= \PhL \nabla_{\ZLpcv} \cvloss \WLT                      & l=1, \dots, L-1 \nonumber \\
\nabla_{\ZLcv} \cvloss &= \sigma^\prime(\ZLcv) \circ \nabla_{\HLcv} \cvloss      &   l=1, \dots, L-1 \nonumber \\
\nabla_{\WL}   \cvloss &= (\PhL  \HLcv)^\top \nabla_{\ZLpcv} \cvloss             & l=0, \dots, L-1. \label{eqn:cvgcn-backprop} 
\end{align}




\begin{lemma}\label{gradient-bound-lemma}
Assume $\sigma(\cdot)$ and $\nabla_z f(y, z)$ are $\rho$-Lipschitz, $\inorm{\nabla_z f(y, z)}\le B$.
Given a fixed dataset $X$ and a sequence of $T$ weights and stochastic propagation matrices $(W_i, \hat P_i)_{i=1}^T$, s.t., 
\begin{enumerate}
	\item $\inorm{W_i}\le B$, $\inorm{\hat P_i}\le B$, and $\inorm{\sigma^\prime(Z_{CV,i})}\le B$,
	\item $\inorm{W_i-W_j}<\epsilon, \forall i, j$,	
\end{enumerate}
let $P=\E \hat P_i$. 
If at time $i$ we feed $(X, W_i, \hat P_i)$ to a GCN with CV estimator to evaluate the prediction for nodes in the minibatch $\Vc_i$,
$$Z_{CV, i}^\bll=\left(\hat P_i^\bl(H_{CV, i}^\bl - \bar H_{CV, i}^\bl) + P\bar H_{CV, i}^\bl\right) W_i^\bl, \quad H_{CV, i}^\bll=\sigma(Z_{CV, i}^\bll).$$
where $\bar H_{CV, i}^\bl$ is the maintained history at time $i$, and $(X, W_i, P)$ to a GCN with exact estimator
$$Z_i^\bll=P H_i^\bl W_i^\bl, \quad H_i^\bll=\sigma(Z_i^\bll),$$
then there exists $K$ that depends on $C$, $B$ and $\rho$
s.t., 
$$\inorm{\E_{\hat P_i, \Vc_i}(W_i) - \nabla \Lc(W_i)} \le K\epsilon, \forall i > LI.$$
\end{lemma}



\begin{proof}
By Lipschitz continuity of $\nabla_z f(y, z)$ and Lemma~\ref{proposition2}, there exists $\dot K$, for all $\hat P_i=(\hat P_i^{(0)}, \dots, \hat P_{i}^{(L-1)})$
\begin{align}
&\inorm{ \nabla_{z^\bL_{CV,v}}f_{CV,v} - \nabla_{z^\bL_v}f_v }\nonumber\\
\le& \rho \inorm{z^\bL_{CV,v} - z^\bL_v} \nonumber\\
\le& \rho \dot K\epsilon,\nonumber\\
\inorm{\sigma^\prime(\ZLcv)-\sigma^\prime(\ZL)} \le& \rho\dot K \epsilon
 \label{eqn:induction-boundary}
\end{align}
We prove by induction that there exists $K_l$, s.t.,
$\forall l\in [L], $, 
\begin{align}\label{eqn:induction-statement}
\inorm{\E_{\hat P^{(\ge l)}} \nabla z_{CV, v}^\bl f_{CV, v} - \nabla z_v^\bl f_v } \le K_l\epsilon, \quad \forall \hat P^{(0)}, \dots, \hat P^{(l-1)},
\end{align}
where $\hat P^{(\ge l)}=(\hat P^{(l)}, \dots, \hat P^{(L-1)})$. By Eq.~(\ref{eqn:induction-boundary}) the statement holds for $l=L$, where $K_L=\rho \dot K$. If the statement holds for $l+1$, i.e., 
$$\inorm{\E_{\hat P^{(\ge l+1)}} \nabla z_{CV, v}^\bll f_{CV, v} - \nabla z_v^\bll f_v } \le K_l\epsilon, \quad \forall \hat P^{(0)}, \dots, \hat P^{(l)},$$
then by Eq.~(\ref{eqn:gcn-backprop}, \ref{eqn:cvgcn-backprop}),
\begin{align*}
&\inorm{\E_{\hat P^{(\ge l)}} \nabla z_{CV, v}^\bl f_{CV, v} - \nabla z_v^\bl f_v } 	 \\
=& \inorm{ 
	\E_{\hat P^{(\ge l)}}  \sigma^\prime(\ZLcv) \circ \PhL \nabla_{\ZLpcv} \cvloss - \sigma^\prime(\ZL) \circ P^{\top} \nabla_{\ZLp} \loss
 }\\
=& \inorm{ \E_{\hat P^{(\ge l)}} \left\{
 \left[
	  \sigma^\prime(\ZLcv) \circ \PhL \nabla_{\ZLpcv} \cvloss \right] - \sigma^\prime(\ZL) \circ P^{\top} \nabla_{\ZLp} \loss 
\right\}}\\
\le& \inorm{ \E_{\hat P^{(\ge l)}} \left\{
\left[
	\left(\sigma^\prime(\ZLcv)-\sigma^\prime(\ZL)\right) \circ \PhL \nabla_{\ZLpcv} \cvloss \right]	
	\right\}} \\
&+\E_{\hat P^{(l)}} \inorm{
	\E_{\hat P^{(\ge l+1)}} \left[
	\sigma^\prime(\ZL) \circ \PhL \left(\nabla_{\ZLpcv} \cvloss - \nabla_{\ZLp} \loss  \right) \right] 
	}  \\
&+\inorm{ \E_{\hat P^{(\ge l)}} \left\{
\left[
	\sigma^\prime(\ZL) \circ \left(\PhL-P^\top\right) \nabla_{\ZLp} \loss  \right]  \right\} }\\
\le&  \E_{\hat P^{(\ge l)}} \left[
	\inorm{\sigma^\prime(\ZLcv)-\sigma^\prime(\ZL)}\inorm{ \PhL \nabla_{\ZLpcv} \cvloss} \right]	
\\
&+\E_{\hat P^\bl}
\inorm{ \sigma^\prime(\ZL) }
\E_{\hat P^{(\ge l+1)}} \inorm{ \PhL }
\E_{\hat P^{(\ge l+1)}} \inorm{ \nabla_{\ZLpcv} \cvloss - \nabla_{\ZLp} \loss  } \\
&+0\\
\le& \rho\dot K \epsilon B^2C^2 + B^2 C^2 K_{l+1} \epsilon \\
=& K_l  \epsilon,
\end{align*}
where $K_l=B^2C^2(\rho\dot K + K_{l+1})$. By induction, Eq.~(\ref{eqn:induction-statement}) holds. Similarly, we can show that there exists $K$, s.t., 
$$\inorm{\E_{\hat P} \nabla_{W^\bl} \cvloss - \nabla_{W^\bl} \loss } < K\epsilon, \quad \forall l\in [L-1].$$
Therefore, 
\begin{align*}
&\inorm{ \E_{\Vc_i, \hat P_i}	g_{CV, i}(W_i) - \nabla \Lc(W_i) }\\
=&\inorm{ \E_{v\in \Vc, \hat P_i}	g_{CV, v}(W_i) - \E_{v\in \Vc}g_v(W_i) }\\
\le&   \E_{\Vc_i} \inorm{ \E_{\hat P_i}g_{CV, v}(W_i) - g_v(W_i) } \\
\le& \E_{\Vc_i} \max_l \inorm{\E_{\hat P} \nabla_{W^\bl} \cvloss - \nabla_{W^\bl} \loss }  \\
\le& K\epsilon. \\
\end{align*}
\end{proof}






\subsection{Proof of Theorem~\ref{M-thm:convergence}}
\begin{reptheorem}{M-thm:convergence}
\convergencethm
\end{reptheorem}

\begin{proof}
This proof is a modification of~\cite{ghadimi2013stochastic}, but using biased stochastic gradients instead. 
We assume the algorithm is already warmed-up for $LI$ steps with the initial weights $W_0$, so that Lemma~\ref{gradient-bound-lemma} holds for step $i>0$. 
Denote $\delta_i = g_{CV,i}(W_i) - \nabla \Lc(W_i)$. By smoothness we have
\begin{align}
\Lc(W_{i+1}) &\le \Lc(W_i) + \iprod{\nabla \Lc(W_i), W_{i+1}-W_{i}} + \frac{\rho}{2}\gamma^2\norm{g_{CV,i}(W_i)}^2_F \nonumber\\
&=\Lc(W_i) - \gamma \iprod{\nabla \Lc(W_i), g_{CV,i}(W_i)} + \frac{\rho}{2}\gamma^2\norm{g_{CV,i}(W_i)}^2_F\nonumber\\
&=\Lc(W_i) - \gamma \iprod{\nabla \Lc(W_i), \delta_i} - \gamma\norm{\nabla \Lc(W_i)}^2 + \frac{\rho}{2}\gamma^2
\left[ \norm{\delta_i}^2 + \norm{\nabla \Lc(W_i)}^2_F + 2\iprod{\delta_i, \nabla\Lc(W_i)} \right] \nonumber\\
&=\Lc(W_i) - (\gamma - \rho\gamma^2) \iprod{\nabla \Lc(W_i), \delta_i} - (\gamma-\frac{\rho\gamma^2}{2}) \norm{\nabla \Lc(W_i)}^2_F + \frac{\rho}{2}\gamma^2\norm{\delta_i}^2_F.\label{eqn:lbound}
\end{align}

For each $i$, consider the sequence of $LI+1$ weights $W_{i-LI}, \dots, W_i$. 
\begin{align*}
&\max_{i-LI\le j, k \le i} \inorm{W_{j}-W_{k}} \le \sum_{j=i-LI}^{i-1} \inorm{W_j-W_{j+1}} \\
=& \sum_{j=i-LI}^{i-1} \gamma \inorm{g_{CV}(W_j)} 
\le \sum_{j=i-LI}^{i-1} \gamma G
= LIG \gamma.
\end{align*}
By Lemma~\ref{gradient-bound-lemma}, there exists $\dot K>0$, s.t.
$$\inorm{\E_{\hat P, \mathcal V_B}\delta_i} = \inorm{\E_{\hat P, \mathcal V_B}g_{CV}(W_i) - \nabla \Lc(W_i)} \le \dot KLIG \gamma, \quad \forall i>0.$$
Assume that $W$ is $D$-dimensional,
\begin{align*}
\E_{\hat P, \mathcal V_B}\iprod{\nabla \Lc(W_i), \delta_i} \le
 D \inorm{\nabla \Lc(W_i)}\inorm{\E_{\hat P, \mathcal V_B} \delta_i} \le \dot KLIDG^2 \gamma \le K \gamma, \\
\E_{\hat P, \mathcal V_B}\norm{\delta_i}^2_F \le D\inorm{g_{CV,i}(W_i)}+D\inorm{\nabla \Lc(W_i)} \le 2DG^2\le K,
\end{align*}
where $K=\max\{\dot KLIDG^2, 2DG^2\}$. Taking $\E_{\hat P, \mathcal V_B}$ to both sides of Eq.~\ref{eqn:lbound} we have
\begin{align*}
\Lc(W_{i+1}) \le \Lc(W_i) + (\gamma- \rho\gamma^2) K\gamma - (\gamma-\frac{\rho\gamma^2}{2}) \norm{\nabla \Lc(W_i)}^2_F + \rho K \gamma^2/2.
\end{align*}
Summing up the above inequalities and re-arranging the terms, we obtain,
\begin{align*}
&(\gamma-\frac{\rho\gamma^2}{2}) \sum_i  \norm{\nabla \Lc(W_i)}^2_F \\
\le& \Lc(W_1) - \Lc(W^*) + K N  (\gamma - \rho\gamma^2) \gamma + \frac{\rho K}{2}N \gamma^2.
\end{align*}
Dividing both sides by $N (\gamma-\frac{\rho\gamma^2}{2})$, and take $\gamma=\min\{\frac{1}{\rho},  \frac{1}{\sqrt{N}}\}$
\begin{align*}
&\E_{R\sim P_R} \norm{\nabla \Lc(W_R)}^2_F \\
\le& 2\frac{\Lc(W_1) - \Lc(W^*) + K N  (\gamma - \rho\gamma^2) \gamma + \frac{\rho K}{2}N \gamma^2}{N \gamma(2-\rho\gamma)}\\
\le& 2\frac{\Lc(W_1) - \Lc(W^*) + K N  (\gamma - \rho\gamma^2) \gamma + \frac{\rho K}{2}N \gamma^2}{N \gamma}\\
\le& 2\frac{\Lc(W_1) - \Lc(W^*)}{N \gamma} + K \gamma(1-\rho\gamma)   + \rho K \gamma\\
\le& 2\frac{\Lc(W_1) - \Lc(W^*)}{\sqrt N} + K \gamma   + \rho K /\sqrt{N}\\
\le& 2\frac{\Lc(W_1) - \Lc(W^*)+K+\rho K}{\sqrt N}.
\end{align*}
Particularly, when $N\rightarrow \infty$, we have $\E_{R\sim P_R} \norm{\nabla \Lc(W_R)}^2_F=0$, which implies that the gradient is asymptotically unbiased.

\end{proof}


==> 93-fastdropout.tex <==




\section{Details of Fast Dropout}
In this section we present the details of applying FastDropout~\citep{wang2013fast} for GCN and CVGCN. FastDropout approximates the activation $H$ of every layer as a Gaussian random variable with known mean and diagonal variance. It approximately computes the mean and variance for each layer analytically. We now describe the update rules by layer. 

\textbf{Input layer:} The input $X$ is treated as a Gaussian random variable with mean $\mu_X=X$ and variance $\Sigma_X=\textbf{0}$. 

\textbf{Dropout layer: } Consider an input random variable $X=\Nc(\muv_X, \diag(\sigmav^2_X))$. The output after applying dropout is $H=\frac{Z}{p}X$, where $Z\sim \mbox{Bern}(p)$. We approximate $H\approx\Nc(\muv_H, \diag(\sigmav_H^2))$, where
\begin{align*}
\muv_H &= \E_Z H = \muv_X \\
\sigmav_H^2 &= \Var_Z H = \frac{\sigmav_X^2 + \muv_X^2}{p} - \muv_X^2.
\end{align*}

\textbf{Linear layer: } Given a Gaussian random variable $X=\Nc(\muv_X, \diag(\sigmav^2_X))$, we apply a linear transformation to it $Z=WX$. The distribution of $Z$ is also Gaussian $Z=\Nc(W\muv_X, W \diag(\sigmav^2_X) W^\top)$. We approximate the covariance $W \diag(\sigmav^2_X) W^\top$ with its diagonal
\begin{align*}
W \diag(\sigmav^2_X) W^\top \approx \diag(W \diag(\sigmav^2_X) W^\top) = \diag(W^2 \sigmav^2_X),
\end{align*}
where $W^2 = W\circ W$. Therefore $Z\approx \Nc(W\muv_X, \diag(W^2\sigmav^2_X))$.

\textbf{Layer normalization: } Given a $D$-dimensional Gaussian random variable $X=\Nc(\muv_X, \diag(\sigmav^2_X))$, we compute the layer normalization~\citep{ba2016layer} as  
\begin{align*}
\mu = \frac{1}{D}\sum_{i=1}^D x_i, \quad \sigma^2 = \frac{1}{D}\sum_{i=1}^D (x_i-\mu)^2, \quad Z=\gamma\frac{X-\mu}{\sigma}+b.
\end{align*}
We approximate the random variable $\mu$ and $\sigma^2$ as constants
\begin{align*}
\hat\mu = \frac{1}{D}\sum_{i=1}^D \mu_{X,i}, \quad \hat\sigma^2=\frac{1}{D}\sum_{i=1}^D (\mu_{X,i}-\hat\mu)^2.
\end{align*}
Then, the random variable after layer normalization is also a Gaussian 
$$Z\approx \Nc(\gamma\frac{\muv_X-\hat\mu}{\hat\sigma}+b, \frac{\gamma^2}{\hat\sigma^2}\diag{\sigmav_X^2}).$$

\textbf{ReLU layer: } For a scalar random variable $X=\Nc(\mu_X, \sigma^2_X)$, its value $Z$ after a ReLU activation $Z=\max\{0, X\}$ is a mixture of a point mass on 0 and a truncated Gaussian distribution. Denote $\alpha=-\frac{\mu_X}{\sigma_X}$, and let $\phi(\cdot)$ and $\Phi(\cdot)$ to be the PDF and CDF of standard normal distribution, respectively. We have 
\begin{align}\label{eqn:relu1}
Z = \begin{cases}
0 & \mbox{with probability }\Phi(\alpha)\\
\Nc(\mu_X, \sigma^2_X | X>0) & \mbox{otherwise},
\end{cases}
\end{align}
where $\Nc(\mu_X, \sigma^2_X | X>0)$ is a truncated normal distribution at $X>0$, whose mean and variance are 
\begin{align}
\E(X | X>0) &= \mu_X + \sigma_X\phi(\alpha)/(1-\Phi(\alpha)), \nonumber\\
\Var(X | X>0) &= \sigma_X^2 \left[1+\alpha\phi(\alpha)/(1-\Phi(\alpha))-\left(\phi(\alpha)/(1-\Phi(\alpha))\right)^2  \right].\label{eqn:relu2}
\end{align}
Combining Eq.~\ref{eqn:relu1} and Eq.~\ref{eqn:relu2} we compute the mean and variance of $Z$
\begin{align}
\E Z &= \mu_X (1-\Phi(\alpha)) + \sigma_X\phi(\alpha),\nonumber\\
\Var Z &= (1-\Phi(\alpha))\Var(X | X>0) + \Phi(\alpha)(1-\Phi(\alpha))(\E Z)^2.\label{eqn:relu3}
\end{align}
Unlike ~\citet{wang2013fast}, who approximate $\Var Z=0$ and solely relies on the next dropout layer to inject noise, we find letting $\Var Z=0$ leads to worse testing accuracy. Therefore we use the true variance as Eq.~\ref{eqn:relu3} and propagate the gradient through it. 


\textbf{Neighbour sampling aggregation layer: } For a random activation matrix $H$, where $H_{vd}=\Nc(\mu_{vd}, \sigma^2_{vd})$, the aggregation $Z=\hat P H$ is just a linear transformation. Same as the linear layer, we can compute the mean and variance of $Z$ as
\begin{align*}
\E_{H} Z_{vd} &= \sum_{v^\prime} \hat P_{v,v^\prime} \mu_{v^\prime,d} \\
\Var_{H} Z_{vd} &=  \sum_{v^\prime} (\hat P_{v,v^\prime})^2 \sigma_{v^\prime, d}^2.
\end{align*}

\textbf{Control variate aggregation layer: } For CVGCN, we have a random activation matrix $H$ as well as a random historical activation matrix $\bar H$, where $H_{vd}=\Nc(\mu_{vd}, \sigma_{vd}^2)$ and $\bar H_{vd}=\Nc(\bar \mu_{vd}, \bar \sigma_{vd}^2)$. We treat $H_{vd}$ and $\bar H_{vd}$ as dependent random variables
\begin{align*}
\epsilon_{vd}\sim \Nc(0, 1), \quad H_{vd}=\mu_{vd}+\sigma_{vd}\epsilon_{vd}, \quad \bar H_{vd}=\bar\mu_{vd}+\bar\sigma_{vd}\epsilon_{vd}.
\end{align*}
CVGCN computes 
\begin{align*}
Z = \hat P(H - \bar H) + P\bar H.
\end{align*}
Then,
\begin{align*}
\E Z_{vd} &= \E \sum_{v^\prime} \left[ \hat P_{v,v^\prime} (H_{v^\prime, d}-\bar H_{v^\prime, d}) + P_{v,v^\prime} \bar H_{v^\prime, d} \right] \\
&=  \sum_{v^\prime} \left[ \hat P_{v,v^\prime} (\Delta\mu_{v^\prime, d}+\Delta\sigma_{v^\prime, d}\E\epsilon_{v^\prime, d}) 
+ P_{v,v^\prime}(\bar\mu_{v^\prime, d}+\bar\sigma_{v^\prime, d}\E\epsilon_{v^\prime, d}) \right]\\
&= \sum_{v^\prime} \left( \hat P_{v,v^\prime} \Delta\mu_{v^\prime, d} + P_{v,v^\prime}\bar\mu_{v^\prime, d} \right),
\end{align*}
where $\Delta\mu_{v^\prime, d}=\mu_{v^\prime, d}-\bar \mu_{v^\prime, d}$ and $\Delta\sigma_{v^\prime, d}=\sigma_{v^\prime, d}-\bar \sigma_{v^\prime, d}$.
\begin{align*}
\Var Z_{vd} &= \E \left\{ \sum_{v^\prime} \left[ \hat P_{v,v^\prime} (H_{v^\prime, d}-\bar H_{v^\prime, d}-\Delta\mu_{v^\prime, d}) + P_{v,v^\prime} (\bar H_{v^\prime, d}-\bar\mu_{v^\prime, d}) \right]\right\}^2 \\
&= \E \left\{ \sum_{v^\prime} \left[ (\hat P_{v,v^\prime} \Delta\sigma_{v^\prime, d} + P_{v,v^\prime} \bar\sigma_{v^\prime, d}) \epsilon_{v^\prime, d} \right] \right\}^2\\
&= \sum_{v^\prime} (\hat P_{v,v^\prime} \Delta\sigma_{v^\prime, d} + P_{v,v^\prime} \bar\sigma_{v^\prime, d})^2.
\end{align*}


Our main purpose of adopting FastDropout is to meet the deterministic activation requirement of CVGCN. Only all the activations before the final control variate aggregation layer need to be deterministic. Therefore, after the final control variate aggregation layer we draw a sample from the approximate Gaussian distribution and use regular dropout for the remaining fully connected layers.







==> 94-variance.tex <==
% !TeX spellcheck = en_US

\section{Derivation of the variance} \label{sec:variance-derivation}
The following proposition is widely used in this section.
\begin{proposition}
Let $X_1, \dots, X_N$ are random variables, then
$$\Var\left[\sum_{i=1}^N X_i\right] = \sum_{i=1}^N\sum_{j=1}^N \Cov\left[X_i, X_j\right].$$ 
\end{proposition}
\begin{proof}
\begin{align*}
\Var\left[\sum_{i=1}^N X_i\right] 
&= \E\left[ \sum_{i=1}^N \sum_{j=1}^N X_i X_j \right] - 
   \left(\E \sum_{i=1}^N X_i\right)^2\\
&= \E\left[ \sum_{i=1}^N \sum_{j=1}^N \left(X_i X_j - \frac{1}{N}\E \sum_{i=1}^N X_i\right)  \right] \\
&= \sum_{i=1}^N\sum_{j=1}^N \Cov\left[X_i, X_j\right].
\end{align*}
\end{proof}

We begin with the proof for the three propositions in the main text.
\begin{repproposition}{M-proposition:var}
\propositionvar
\end{repproposition}
\begin{proof}
We denote the $D^\bl$ samples in the set as $v_1, \dots, v_{D^\bl}$.Let $\bar x = \frac{1}{n(u)}\sum_{v\in \nv(u)}x_v$, then
\begin{align*}
&\Var_{\hat \nv^\bl(u)}\left[\frac{n(u)}{D^\bl}\sum_{v\in \hat \nv^\bl(u)} x_v \right]\\
=& \Var_{v_1, \dots, v_{D^\bl}}\left[\frac{n(u)}{D^\bl}\sum_{i=1}^{D^\bl} x_{v_i} \right]\\
=& \left(\frac{n(u)}{D^\bl}\right)^2 \sum_{i=1}^{D^\bl}  \sum_{j=1}^{D^\bl}
\Cov_{v_1, \dots, v_{D^\bl}}\left[x_{v_i}, x_{v_j}\right] \\
=& \left(\frac{n(u)}{D^\bl}\right)^2\left\{
\sum_{i=1}^{D^\bl} \Var_{v_i} \left[x_{v_i}^2\right]  + 
\sum_{i\ne j} \Cov_{v_i, v_j}\left[x_{v_i}, x_{v_j}\right]
\right\}\\
=& \left(\frac{n(u)}{D^\bl}\right)^2\left\{
\frac{D^\bl}{n(u)}\sum_{v\in \nv(u)} (x_v - \bar x)^2 +
\frac{D^\bl(D^\bl-1)}{n(u)(n(u)-1)} \left[\sum_{i, j\in \nv(u)} (x_i-\bar x)(x_j-\bar x) - \sum_{i\in \nv(u)} (x_i-\bar x)^2 \right]\right\}\\
=& \frac{n(u)}{D^\bl} \left(1-\frac{D^\bl-1}{n(u)-1}\right) \left(
\sum_{v\in \nv(u)} x_v^2 - n(u)\bar x^2
\right) \\
=& \frac{1}{2D^\bl}\left(1-\frac{D^\bl-1}{n(u)-1}\right) \left(2n(u)\sum_{v\in \nv(u)} x_v^2 - \sum_{v_1, v_2\in \nv(u)} 2 x_{v_1} x_{v_2} 
\right)\\
=& \frac{C_u^\bl}{2D^\bl} \sum_{v_1, v_2\in \nv(u)} (x_{v_1}-x_{v_2})^2.
\end{align*}
\end{proof}

\begin{repproposition}{M-proposition-varr}
\propositionvarr
\end{repproposition}
\begin{proof}
\begin{align*}
&\Var_{X, \hat \nv^\bl(u)}\left[\frac{n(u)}{D^\bl}\sum_{v\in \hat \nv^\bl(u)} x_v \right]\\
=& \left(\frac{n(u)}{D^\bl}\right)^2
\E_X  \left\{ \sum_{i=1}^{D^\bl} \E_{\snbr} x_{v_i}^2 + \sum_{i\ne j} \E_{\snbr} x_{v_i} x_{v_j}  \right\}\\
=& \left(\frac{n(u)}{D^\bl}\right)^2 
\E_X  \left\{
\frac{D^\bl}{n(u)} \sum_{i\in\nbr} x_{i}^2 + 
\frac{D^\bl(D^\bl-1)}{n(u)(n(u)-1)} \sum_{i, j\in \nbr, i\ne j} x_i x_j
 \right\}\\
=& \frac{n(u)}{D^\bl} \sum_{i\in \nbr}\var{}{x_i}.
%\frac{1}{2D^\bl} \var{X}{\sum_{v_1, v_2\in \nv(u)} (x_{v_1}-x_{v_2})^2} \\
%=& \frac{1}{2D^\bl} \left(2 n(u)\sum_{v\in\nbr} \E x_v^2 -2 \sum_{v1, v2\in \nbr, v1\ne v2} \E x_{v_1}x_{v_2} \right) \\
%=&\frac{n(u)}{D^\bl} \sum_{v\in\nbr}\var{}{x_v}.
\end{align*}
\end{proof}

\begin{repproposition}{M-proposition-varsum}
\propositiontworv
\end{repproposition}
\begin{proof}
\begin{align*}
\Var_{X, Y}\left[f(X, Y) + g(Y)\right]=\Var_{X, Y} f(X, Y) + \Var_Y g(Y) + 2\Cov_{X,Y}[f(X, Y), g(Y)],
\end{align*}
where 
\begin{align*}
\Cov_{X,Y}[f(X, Y), g(Y)] 
&= \E_Y \E_X \left[ (f(X, Y) - \E_{X,Y} f(X, Y))(g(Y) - E_Y g(Y))  \right]\\
&= \E_Y  \left[ (\E_X f(X, Y) - 0)(g(Y) - E_Y g(Y)) 
\right] \\
&= \E_Y \left[ 0(g(Y) - E_Y g(Y)) \right] = 0.
\end{align*}
\end{proof}

Then, we derive the variance of the estimators with dropout is present.
\subsection{Variance of the exact estimator}
\begin{align*}
\var{M}{\sum_{v\in \nv(u)} P_{uv}h_v^\bl}=
\var{M}{\sum_{v\in \nv(u)} P_{uv}\rh_v^\bl} = \sum_{v\in \nv(u)} P_{uv}^2\var{M}{\rh_v^\bl} = S_u^\bl.
\end{align*}

\subsection{Variance of the NS estimator}
\begin{align*}
&\var{\snbr, M}{\NS_u^\bl} \\
=& \var{\snbr, M}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} h_v^\bl
}\\
=& \var{\snbr, M}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} (\rh_v^\bl +\mu_v^\bl )
}\\
=& \var{\snbr, M}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} \rh_v^\bl
} + \var{\snbr}{
\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} \mu_v^\bl
},
\end{align*}
where the last equality is by Proposition~\ref{M-proposition-varsum}. By Proposition~\ref{M-proposition-varr}, VD is
\begin{align*}
&\var{\snbr, M}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} \rh_v^\bl
}\\
=&\Var_M \var{\snbr}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} \rh_v^\bl
}\\
=& \frac{n(u)}{D^\bl}S_u^\bl ,
\end{align*}
where $S_u^\bl=\sum_{v\in \nbr}\var{M}{P_{uv} h_{v}^\bl}$ is defined in Sec.~\ref{M-sec:variance-analysis}. By Proposition~\ref{M-proposition:var}, VNS is
\begin{align*}
\var{\snbr}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} \mu_v^\bl
} =  \frac{C_u^\bl}{2D^\bl}\sum_{v_1, v_2\in \nbr} (P_{uv_1} \mu_{v_1}^\bl - P_{uv_2} \mu_{v_2}^\bl)^2.
\end{align*}


\subsection{Variance of the CVD estimator}


\begin{align*}
&\var{\snbr, M}{\CVD_u^\bl} \\
=& \var{\snbr, M}{
\sqrt{\frac{n(u)}{D^{(l)}}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \rh^\bl_v  + 
\frac{n(u)}{D^{(l)}}   \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \mu^\bl_v + 
\sum_{v\in \nv(u)} P_{uv}\bar\mu^\bl_v
}\\
=& \var{\snbr, M}{
	\sqrt{\frac{n(u)}{D^{(l)}}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \rh^\bl_v} + 
\var{\snbr}{
\frac{n(u)}{D^{(l)}}   \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \mu^\bl_v + 
\sum_{v\in \nv(u)} P_{uv}\bar\mu^\bl_v
},
\end{align*}
where the last equality is by Proposition~\ref{M-proposition-varsum}. By Proposition~\ref{M-proposition-varr}, VD is
\begin{align*}
&\var{\snbr, M}{
	\sqrt{\frac{n(u)}{D^\bl}}\sum_{v\in\snbr} P_{uv} \rh_v^\bl
}\\
=&\frac{D^\bl}{n(u)} \Var_M \var{\snbr}{
	\frac{n(u)}{D^\bl}\sum_{v\in\snbr} P_{uv} \rh_v^\bl
}\\
=& S_u^\bl .
\end{align*}
By Proposition~\ref{M-proposition:var}, VNS is
\begin{align*}
&\var{\snbr}{
	\frac{n(u)}{D^{(l)}}   \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \mu^\bl_v + 
	\sum_{v\in \nv(u)} P_{uv}\bar\mu^\bl_v
} \\
=& 
\var{\snbr}{
	\frac{n(u)}{D^{(l)}}   \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \mu^\bl_v 
}\\
 =&  \frac{C_u^\bl}{2D^\bl}\sum_{v_1, v_2\in \nbr} (P_{uv_1} \Delta \mu_{v_1}^\bl - P_{uv_2} \Delta \mu_{v_2}^\bl)^2.
\end{align*}



\subsection{Variance of the CV estimator}
\begin{align*}
	&\var{\snbr, M}{\CV_u^\bl} \\
	=& \var{\snbr, M}{
		\frac{n(u)}{D^{(l)}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta h^\bl_v  + 
		\sum_{v\in \nv(u)} P_{uv}\bar h^\bl_v
	}\\
	=& \var{\snbr, M}{
		\frac{n(u)}{D^{(l)}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \rh^\bl_v  + 
		\sum_{v\in \nv(u)} P_{uv}\bar \rh^\bl_v
		+
		\frac{n(u)}{D^{(l)}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \mu^\bl_v  + 
		\sum_{v\in \nv(u)} P_{uv}\bar \mu^\bl_v
	}\\
	=& \var{\snbr, M}{
		\frac{n(u)}{D^{(l)}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \rh^\bl_v  + 
		\sum_{v\in \nv(u)} P_{uv}\bar \rh^\bl_v} \\
	&+ \var{\snbr}{\frac{n(u)}{D^{(l)}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \mu^\bl_v  + 
		\sum_{v\in \nv(u)} P_{uv}\bar \mu^\bl_v},
\end{align*}
where $\Delta\rh_v^{(l)} = (h_v^\bl - \mu_v^\bl) - (\bar h_v^\bl - \bar \mu_v^\bl)$, and the last equality is by Proposition~\ref{M-proposition-varsum}. The VNS term is the same with CVD's VNS term.

To analyze the VD, we further assume $\bar \rh_v^\bl$ and $\rh_v^\bl$ are i.i.d., so $\E_M \Delta \rh_v^\bl = 0$, $\E_M (\Delta \rh_v^\bl)^2 = 2 \E_M (\rh_v^\bl)^2$, and $\E_M \rh_v^\bl \Delta \rh_v^\bl = \E_M (\rh_v^\bl)^2$. 
\begin{align*}
&\var{\snbr, M}{
	\frac{n(u)}{D^{(l)}} \sum_{v\in \hat\nv^\bl (u)} P_{uv} \Delta \rh^\bl_v  + 
	\sum_{v\in \nv(u)} P_{uv}\bar \rh^\bl_v}  \\
=& \E_{\snbr, M} \Big\{
\left(\frac{n(u)}{D^\bl}\right)^2 \sum_{i,j\in \snbr}P_{ui}P_{uj}\Delta\rh_{i}^\bl \Delta\rh_{j}^\bl + 
\sum_{i,j\in \nbr} P_{ui}P_{uj} \bar\rh_i^\bl\bar\rh_j^\bl \\
&+ 2\frac{n(u)}{D^\bl} \sum_{i\in \snbr, j\in \nbr}P_{ui}P_{uj}\Delta\rh_i^\bl\bar\rh_j^\bl
\Big\}\\
=& 
\left(\frac{n(u)}{D^\bl}\right)^2 \sum_{i\in \snbr}\E_{\snbr, M} (P_{ui}\Delta\rh_i^\bl)^2 + \sum_{i\in \nbr}P_{ui}^2 \E_M\bar\rh_i^\bl
+ 2\sum_{ij\in \nbr} P_{ui}P_{uj}\Delta\rh_i^\bl\bar\rh_j^\bl\\
=& \frac{n(u) }{D^\bl } \sum_{i\in \nbr} P_{ui^2} \E_M  (\rh_i^\bl)^2 + \sum_{i\in \nbr}P_{ui}^2 \E_M\bar\rh_i^\bl +  2\sum_{i\in \nbr}P_{ui}^2 \E_M\bar\rh_i^\bl \\
=& \left(3+\frac{n(u)}{D^\bl}\right) S_u^\bl.
\end{align*}





==> 95-experiment-setup.tex <==
% !TeX spellcheck = en_US
\section{Experiment setup}\label{sec:experimental-setup}
In this sections we describe the details of our model architectures. We use the Adam optimizer~\cite{kingma2014adam} with learning rate 0.01. 
\begin{itemize}
    \item Citeseer, Cora, PubMed and NELL: We use the same architecture as~\cite{kipf2016semi}: two graph convolution layers with one linear layer per graph convolution layer. We use 32 hidden units, 50\% dropout rate and $5\times 10^{-4}$ L2 weight decay for Citeseer, Cora and PubMed and 64 hidden units, 10\% dropout rate and $10^{-5}$ L2 weight decay for NELL. 
    \item PPI and Reddit: We use the mean pooling architecture GraphSAGE-mean proposed by~\cite{hamilton2017inductive}. We use two linear layers per graph convolution layer. We set weight decay as zero, dropout rate as 20\%, and adopt layer normalization~\cite{ba2016layer} after each linear layer. We use 512 hidden units for PPI and 128 hidden units for Reddit. We find that our architecture can reach 97.8\% testing micro-F1 on the PPI dataset, which is significantly higher than 59.8\% reported by~\cite{hamilton2017inductive}. We find the improvement is from wider hidden layer, dropout and layer normalization. 
\end{itemize}

==> 96-pseudocode.tex <==
% !TeX spellcheck = en_US
\section{Pseudocode}\label{sec:pseudocode}

\begin{algorithm}[t]
	\caption{Constructing the receptive fields and random propagation matrices. \label{alg:rf}}
	\begin{algorithmic}
		\State $\rv^\bL \leftarrow \Vc_B$
		\For {layer $l\leftarrow L-1$ \mbox{ to } 0}
			\State $\rv^\bl \leftarrow \varnothing$
			\State $\hat P^\bl \leftarrow \mathbf{0}$
			\For {each node $u \in \rv^\bll$}
				\State $\rv^\bl \leftarrow \rv^\bl\cup \{u\}$
				\State $\hat P^\bl_{uu} \leftarrow \hat P^\bl_{uu} +  P_{uu} n(u)  / D^\bl $
				\For {$D^\bl-1$ random neighbors $v\in \nv(u)$}
					\State $\rv^\bl \leftarrow \rv^\bl\cup \{v\}$
					\State $\hat P^\bl_{uv} \leftarrow \hat P^\bl_{uv} +  P_{uv} n(u)  / D^\bl$				
				\EndFor
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
	\caption{Training with the CV algorithm\label{alg:cv}}
	\begin{algorithmic}
		\For {each minibatch $\mathcal V_B\subset \mathcal V$}
		\State Compute the receptive fields $\rv^\bl$ and stochastic propagation matrices $\hat P^\bl$ as Alg.~\ref{alg:rf}.
		\State (Forward propgation)
		\For {each layer $l\leftarrow 0$ \mbox{ to } $L-1$}
		\State $Z^{(l+1)}\leftarrow \left(\hat P^{(l)}(H^{(l)}-\bar H^{(l)} + P \bar H^{(l)}\right) W^{(l)}$
		\State $H^{(l+1)}\leftarrow\sigma(Z^{(l+1)})$
		\EndFor
		\State Compute the loss $\Lc=\frac{1}{|\mathcal V_B|}\sum_{v\in \mathcal V_B} f(y_v, Z^{(L)}_v)$
		\State (Backward propagation)
		\State $W\leftarrow W - \gamma_i \nabla_W \Lc$
		\State (Update historical activations)
		\For {each layer $l\leftarrow 0$ \mbox{ to } $L-1$}
		\For {each node $v\in \rv^\bl$}
		\State $\bar h_v^\bl \leftarrow h_v^\bl$
		\EndFor
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}
	\caption{Training with the CVD algorithm\label{alg:cvd}}
	\begin{algorithmic}
		\For {each minibatch $\mathcal V_B\subset \mathcal V$}
		\State Compute the receptive fields $\rv^\bl$ and stochastic propagation matrices $\hat P^\bl$ as Alg.~\ref{alg:rf}.
		\State (Forward propgation)
		\For {each layer $l\leftarrow 0$ \mbox{ to } $L-1$}
		\State $U\leftarrow \left( \bar P^{(l)}(H^{(l)}-\mu^{(l)}) +\hat P^{(l)}(\mu^{(l)}-\bar\mu^{(l)}) + P \bar H^{(l)}\right)$
		\State $H^{(l+1)}\leftarrow\sigma(\mbox{Dropout}_p(U)W^{(l)})$
		\State $\mu^{(l+1)}\leftarrow\sigma(UW^{(l)})$		
		\EndFor
		\State Compute the loss $\Lc=\frac{1}{|\mathcal V_B|}\sum_{v\in \mathcal V_B} f(y_v, H^{(L)}_v)$
		\State (Backward propagation)
		\State $W\leftarrow W - \gamma_i \nabla_W \Lc$
		\State (Update historical activations)
		\For {each layer $l\leftarrow 0$ \mbox{ to } $L-1$}
		\For {each node $v\in \rv^\bl$}
		\State $\bar h_v^\bl \leftarrow h_v^\bl$
		\EndFor
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}


As mentioned in Sec.~\ref{M-sec:implementation}, an iteration of our algorithm consists the following operations:
\begin{enumerate}
	\item Randomly select a minibatch $\mathcal V_B\in \mathcal V_L$ of nodes;
	\item Build a computation graph that only contains the activations $h_v^\bl$ and $\bar h_v^\bl$ needed for the current minibatch;
	\item Get the predictions by forward propagation as Eq.~(\ref{eqn:zupdate});
	\item Get the gradients by backward propagation, and update the parameters by SGD;
	\item Update the historical activations.
\end{enumerate}
For step 2, we construct the receptive fields $\rv^\bl$ and stochastic propagation matrices $\hat P^\bl$ as Alg.~\ref{alg:rf}.



\subsection{Training with the CV estimator}
Alg.~\ref{alg:cv} depicts the training algorithm using the CV estimator. We perform forward propagation according to Eq.~(\ref{M-eqn:zupdate}), compute the stochastic gradient, and then update the historical activations $\bar H^{(l)}$ for all the nodes in $\rv^\bl$. Let $W=(W^{(0)}, \dots, W^{(L-1)})$ be all the trainable parameters, the gradient $\nabla_W \Lc$ is computed automatically by frameworks such as TensorFlow.


\subsection{Training with the CVD estimator}
Training with the CVD estimator is similar with the CV estimator, except it runs two versions of the network, with and without dropout, to compute the samples $H$ and their mean $\mu$ of the activation. The matrix $\bar P_{uv}^\bl=\hat P_{uv}^\bl / \sqrt{n(v)}$ , where $n(v) $ is the degree of node $v$. 


==> 97-more-layers.tex <==
% !TeX spellcheck = en_US
\section{Experiment for 3-layer GCNs}

We test 3-layer GCNs on the Reddit dataset. The settings are the same with 2-layer GCNs in Sec.~\ref{M-sec:convergence-dropout}. To ensure M1+PP can run in a reasonable amount of time, we subsample the graph so that the maximum degree is 10. The convergence result is shown as Fig.~\ref{fig:iter-acc-3}, where the conclusion is similar with the two-layer models: CVD+PP is the best-performing approximate algorithm, followed by CV+PP, and then NS+PP and NS.  The time consumption to reach 0.94 testing accuracy is shown in Table~\ref{tbl:time3}.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/reddit3_0_iter_acc.pdf}
	\includegraphics[width=\linewidth]{figures/legend_0.pdf}
	\caption{Comparison of validation accuracy with respect to number of epochs for 3-layer GCNs. }
	\label{fig:iter-acc-3}
\end{figure}


\begin{table}[t]
	\caption{Time to reach 0.95 testing accuracy.}\label{tbl:time3}
	\centering
\begin{tabular}{c|ccccc}
	\hline
	\multirow{2}{*}{Alg.}     & Valid. & \multirow{2}{*}{Epochs} & Time &  Sparse & Dense \\
	& acc. &  & (s) &  GFLOP & TFLOP \\
	\hline
Exact & 0.940 & \textbf{3.0} & 199 & 306 & 11.7\\
NS & 0.940 & 24.0 & 148 & 33.6 & 9.79\\
NS+PP & 0.940 & 12.0 & 68 & \textbf{2.53} & 4.89\\
CV+PP & 0.940 & 5.0 & \textbf{32} & 8.06 & \textbf{2.04}\\
CVD+PP & 0.940 & 5.0 & 36 & 16.1 & 4.08\\
	\hline
\end{tabular}
\end{table}

==> 98-independent-gaussian.tex <==
% !TeX spellcheck = en_US
\section{Correlation between node activations}\label{sec:indep-gaussian}
In our analysis of the variance for the CVD estimator in Sec.~\ref{M-sec:variance-analysis}, we assume that the activations for different nodes are uncorrelated, i.e., $\Cov_{M}\left[ h_u^\bl, h_v^\bl \right]=0$, for all $u\ne v$, where $M$ is the dropout mask. We show the rationale behind this assumption in this section. For 2-layer GCNs, the activations are indeed independent, and the correlation is still weak for deeper GCNs due to the sparsity of our sampled graph.
\subsection{Results for 2-layer GCNs}\label{sec:2-layer}
For a 2-layer GCN with the first layer pre-processed, the activations of nodes are independent. Suppose we want to compute the prediction for a node on the second layer. Without loss of generality, assume that we want to compute $z^{(2)}_1$, and the neighbors of node 1 are $1, \dots, D$. 
The activation $h_v^{(1)}=\sigma\left( (M_v\circ u_v^{(0)})W^{(0)}\right)$, where $u_v^{(0)}=(PH^{(0)})_v$ is a random variable with respect to $M_v$,  $M_v\sim \mbox{Bernoulli}(p)$ is the dropout mask. We show that $h_v^{(1)}$ and $h_{v^\prime}^{(1)}$ are independent, for $v\ne v^\prime$ by the following lemma.
\begin{lemma}
	If $a$ and $b$ are independent random variables, then their transformations $f_1(a)$ and $f_2(b)$ are independent. 
\end{lemma}
Because for any event $A$ and $B$, $P(f_1(a)\in f_1(A), f_2(b)\in f_2(B))=P(a\in A, b\in B)=P(a\in A)P(b\in B)=P(f_1(a)\in f_1(A))P(f_2(B)\in f_2(B))$, where $f_1(A)=\{f_1(a) | a\in A\}$ and $f_2(B)=\{f_2(b) | b\in B\}$. 

Let $h_v^{(1)}=f_1(M_v):=\sigma\left((M_v\circ u_v^{(0)})W^{(0)}\right)$ and $h_{v^\prime}^{(1)}=f_1(M_{v^\prime}):=\sigma\left((M_{v^\prime}\circ u_{v^\prime}^{(0)})W^{(0)}\right)$, because $M_v$ and $M_{v^\prime}$ are independent Bernoulli random variables, $h_v^{(1)}$ and $h_{v^\prime}^{(1)}$ are independent.

The result can be further generalized to deeper models. If the receptive fields of two nodes does not overlap, they should be independent. 

\subsection{Empirical results for deeper GCNs}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\linewidth]{figures/correlation_citeseer.pdf}
	\includegraphics[width=0.45\linewidth]{figures/correlation_cora.pdf}
	\includegraphics[width=0.45\linewidth]{figures/correlation_pubmed.pdf}
	\includegraphics[width=0.45\linewidth]{figures/correlation_ppi.pdf}
	\caption{Average feature and neighbor correlations in a 10-layer GCN.\label{fig:correlation}}
\end{figure}

Because we only sample two neighbors per node, the sampled subgraph is very close to a graph with all its nodes isolated, which reduces to the MLP case that~\cite{wang2013fast} discuss. 

We empirically study the correlation between feature dimensions and neighbors. The definition of the correlation between feature dimensions is the same with~\cite{wang2013fast}. For each node $v$ on layer $l$, we compute the correlation between each feature dimension of $h^{(l)}_v$
\begin{align*}
\mbox{Cov}^{(l,v)}_{ij} &:= \mathbb{C}[h^{(l)}_{vi}, h^{(l)}_{vj}]\\
\mbox{Corr}^{(l,v)}_{ij} &:= \frac{\mbox{Cov}^{(l,v)}_{ij}}{\sqrt{\mbox{Cov}^{(l,v)}_{ii}}\sqrt{\mbox{Cov}^{(l,v)}_{jj}}},\nonumber
\end{align*}
where $i$ and $j$ are the indices for different hidden dimensions, and $\mathbb C[X, Y]=\E[(X-\E X)(Y-\E Y)]$ is the covariance between two random variables $X$ and $Y$. We approximate $\mbox{Cov}^{(l,v)}_{ij}$ with 1,000 samples of the activations $h^{(l)}_{vi}$ and $h^{(l)}_{vj}$, by running the forward propagation 1,000 times with different dropout masks.
 We define the \emph{average feature correlation on layer $l$} to be $\mbox{Cov}^{(l,v)}_{ij}$ averaged by the nodes $v$ and dimension pairs $i\ne j$.


To compute the correlation between neighbors, we treat each feature dimension separately. 
For each layer $l+1$, node $v$, and dimension $d$, we compute the correlation matrix of all the activations  $\{h^{(l)}_{id} | i\in \bar\nv^{(l)}(v)\}$ that are needed by $h^{(l+1)}_{vd}$, where $\bar\nv^{(l)}(v)=\{i | \hat P^{(l)}_{vi}\ne 0\}$ is the set of subsampled neighbors for node $v$:
\begin{align*}
\mbox{Cov}^{(l,v,d)}_{ij} &:= \mathbb{C}[h^{(l)}_{id}, h^{(l)}_{jd}]\\
\mbox{Corr}^{(l,v,d)}_{ij} &:= \frac{\mbox{Cov}^{(l,v,d)}_{ij}}{\sqrt{\mbox{Cov}^{(l,v,d)}_{ii}}\sqrt{\mbox{Cov}^{(l,v,d)}_{jj}}},\nonumber
\end{align*}
where the indices $i, j \in \bar\nv^{(l)}(v)$. 
Then, we compute the average correlation of all pairs of neighbors $i\ne j$.
\begin{align*}
\mbox{AvgCorr}^{(l,v,d)} &:= \frac{1}{\abs{\bar\nv^{(l)}(v)} (\abs{\bar\nv^{(l)}(v)} - 1)} \sum_{i\ne j} \mbox{Corr}^{(l,v,d)}_{ij},
\end{align*}
and define the \emph{average neighbor correlation on layer $l$} as $\mbox{AvgCorr}^{(l,v,d)}$ averaged over all the nodes $v$ and dimensions $d$.

We report the average feature correlation and the average neighbor correlation per layer, on the Citeseer, Cora, PubMed and PPI datasets. These quantities are too expensive to compute for NELL and Reddit. On each dataset, we train a GCN with 10 graph convoluation layers until early stopping criteria is met, and compute the average feature correlation and the average neighbor correlation for layer 1 to 9. We are not interested in the correlation on layer 10 because there are no more graph convolutional layers after it. The result is shown as Fig.~\ref{fig:correlation}. As analyzed in Sec.~\ref{sec:2-layer}, the average neighbor correlation is close to zero on the first layer, but it is not exactly zero due to the finite sample size for computing the empirical covariance. There is no strong tendency of increased correlation as the number of layers increases, after the third layer. 
The average neighbor correlation and the average feature correlation remain on the same order of magnitude, so bringing correlated neighbors does not make the activations much more correlated than the MLP case~\cite{wang2013fast}. 
Finally, both correlations are much smaller than one.




==> listofitems.tex <==
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.51}                              %
%                                                                    %
\def\loidate                  {2017/10/24}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% --------------------------------------------------------------------
% Author     : Christian Tellechea, Steven B. Segletes
% Status     : Maintained
% Maintainer : Christian Tellechea
% Email      : unbonpetit@netc.fr
%              steven.b.segletes.civ@mail.mil
% Package URL: https://www.ctan.org/pkg/listofitems
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2017
% Licence    : Released under the LaTeX Project Public License v1.3c
%              or later, see http://www.latex-project.org/lppl.txt
% Files      : 1) listofitems.tex
%              2) listofitems.sty
%              3) listofitems-fr.tex
%              4) listofitems-fr.pdf
%              5) listofitems-en.tex
%              6) listofitems-en.pdf
%              7) README
% --------------------------------------------------------------------
\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% v\'erification de la pr`'esence de etex %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\expandafter\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---- macros de d\'eveloppement et de manipulation d'arguments
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_i\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_i#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_i\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_i#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_i{#1}}
\def\loi_argcsname_i#1#2{\loi_expafter{#1}{\csname#2\endcsname}}

%--- macros de test
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_i{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_i}
\long\def\loi_ifprimitive#1{\edef\loi_tempa{\meaning#1}\edef\loi_tempb{\string#1}\loi_ifx{\loi_tempa\loi_tempb}}
\long\def\loi_ifcs#1{% #1 est-il une sc (n'\'etant pas une primitive) ?
	\loi_ifempty{#1}
		\loi_second% si #1 est vide, faux
		{\loi_ifspacefirst{#1}
			\loi_second% si espace en 1er, faux
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup \escapechar`\_
					\if\expandafter\loi_firsttonil\detokenize{#1}\_nil\expandafter\loi_firsttonil\string\relax\_nil
						\loi_ifprimitive{#1}
							{\endgroup\expandafter\loi_second}
							{\endgroup\expandafter\loi_first}%
					\else
						\endgroup\expandafter\loi_second
					\fi
				}
				\loi_second% si plusieurs tokens, faux
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}

%--- macro de type for
%      Voir codes 150 \`a 155 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 175 \`a 184 du livre "Apprendre \`a programmer en TeX"
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\expandafter\loi_fornum_i\csname loi_fornum_\string#1\expandafter\endcsname\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_i#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%--- macros retirant les espaces extr\^emes
%      Voir codes 320 \`a 324 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 339 \`a 343 de "Apprendre \`a programmer en TeX"
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_i\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_i#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_i}
\long\def\loi_removefirstspaces_i#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_i\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_i#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_i#1 ^^00{\loi_removelastspaces_ii#1^^00}
\long\def\loi_removelastspaces_ii#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_i#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte o\`u les espaces extr\^emes sont retir\'es
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_i}
\def\setsepchar_i{\loi_ifx{[\loi_nxttok}\setsepchar_ii{\setsepchar_ii[/]}}
\long\def\setsepchar_ii[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_ii[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % r\'einitaliser niveau initial \`a 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_iv1{,}%
			}
			{\readlist_iv1{#2}}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de s\'eparation
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_i1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_i#1#2#3#4#5,{% #1=compteur de profondeur #2=index pr\'ec\'edents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_iii#2\loi_quark}% supprimer la derni\`ere virgule
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}}% si profondeur trop grande
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_ii{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_ii#1#2#3{\loi_exparg\loi_normalizeindex_i{\number\numexpr#2+1}{#3#1,}}% #1=index \`a rajouter  #2=compteur de profondeur #3=index pr\'ec\'edents
\def\loi_normalizeindex_iii#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_i{#1},}\loi_invalidindex_i{#1}{#2}}
\def\loi_invalidindex_i#1#2{\loi_invalidindex_ii#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_ii#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignor\'es

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{%
	\let\loi_def\gdef \let\loi_edef\xdef \def\loi_let{\global\let}%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\loi_let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\def\readlist{%
	\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\long\def\readlist_i#1#2{% #1=macro stockant les \'el\'ements  #2=liste des \'el\'ements
	\loi_ifcs{#2}
		{\loi_exparg{\readlist_i#1}{#2}}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste enti\`ere
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% s\'eparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_ii{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_auxmacrolistitem#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_ii{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_iii\loi_currentsep||\_nil
}
\long\def\readlist_iii#1||#2\_nil#3{\readlist_iv1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un \'el\'ement vide pour le test ifempty ci dessous
\long\def\readlist_iv#1#2{% #1=compteur d'index  #2=liste d'\'el\'ements \`a examiner
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_vi{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}}% aller isoler le 1er item
}
\long\def\readlist_v#1#2{\readlist_vi{#2}{}#1||\loi_quark||#2\_nil}% #1=liste s\'eparateurs (s\'ep=||)  #2=chaine de tokens
\long\def\readlist_vi#1#2#3||{% #1=liste restante   #2=dernier <sep utile>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}
		{\loi_ifempty{#2}% si #1 vide, aucun <sep utile> n'a \'et\'e trouv\'e, il reste \`a lire "<liste compl\`ete>\_nil"
			{\long\def\readlist_vii##1\_nil##2{\loi_exparg{\readlist_ix{##2}{}}{\loi_gobarg##1}{#2}}}% ##2=compteur d'index
			{\long\def\readlist_vii##1#2{\loi_exparg\readlist_viii{\loi_gobarg##1}\relax}%
			\long\def\readlist_viii##1##2\_nil##3{\loi_exparg{\readlist_ix{##3}}{\loi_gobarg##2}{##1}{#2}}% ##3=compteur d'index
			}%
		\readlist_vii\relax% le \relax meuble l'argument d\'elimit\'e
		}
		{\long\def\readlist_vii##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_vi{#1}{#2}}% recommencer avec le m\^eme <sep utile>
				{\readlist_vi{##1#3}{#3}}% sinon raccourcir <liste restante> et <sep courant>:=<sep utile>
			}%
		\readlist_vii#1#3\_nil
		}%
}
\long\def\readlist_ix#1#2#3{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extr\^emes
		{\loi_exparg{\loi_exparg{\readlist_x{#1}{#2}}}{\loi_removeextremespaces{#3}}}% red\'efinir l'\'el\'ement courant
		{\readlist_x{#1}{#2}{#3}}%
}
\long\def\readlist_x#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant   #4=sep utilis\'e
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_iv{#1}{#2}}% si l'on n'ignore pas les \'el\'ements vides :
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel \`a la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel \`a la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_ii{#3}% recommencer avec l'\'el\'ement courant
			}
			{}%
		\loi_exparg\readlist_iv{\number\numexpr#1+1}{#2}% puis chercher l'\'el\'ement suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_i{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_i#1#2{% #1=macro name   #2=index non normalis\'e    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_ii\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_ii#1#2#3{% #1=err   #2=index normalis\'e  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_i{\noexpand\foreachitem_iii\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_ii
}
\def\foreachitem_ii{\loi_ifx{\loi_nxttok[}\foreachitem_i{\foreachitem_i[]}}
\def\foreachitem_iii#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_iv\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_iv#1#2{\loi_ifempty{#2}{\foreachitem_v{#1}{}}{\foreachitem_v{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_v#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associ\'e  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_i}{\let\showitems_cmd\loi_identity\showitems_i}}
\def\showitems_i#1{\def\showitems_ii{\showitems_iv#1}\futurelet\loi_nxttok\showitems_iii}
\def\showitems_iii{\loi_ifx{\loi_nxttok[}\showitems_ii{\showitems_ii[]}}
\def\showitems_iv#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % r\'eglages identiques \`a LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir codes 251 \`a 254 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
		\hbox{% et pages 271 \`a 274 de "Apprendre \`a programmer en TeX"
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par d\'efaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_i#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% r\'eglages par d\'efaut %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
#                             Historique                             #
######################################################################

v1.0  19/8/2016
      - Premi\`ere version publique

v1.1  01/09/2016
      - Stockage des s\'eparateurs dans <macrolist>sep
      - bug corrig\'e dans \loi_restorecatcode

v1.2  22/10/2016
      - macros \greadlist et \gitemtomacro pour la globalit\'e

v1.3  18/11/2016
      - bugs corrig\'es dans la gestion de la globalit\'e

v1.4  05/10/2017
      - test \loi_ifprimitive ajout\'e au test \loi_ifcs
      - suppression de \loi_expafternil, cr\'eation de \loi_expafter,
        modification de \loi_argcsname
      - correction d'un bug : \setsepchar{\par} ne provoque plus
        d'erreur. \loi_ifnum devient \long

v1.5  06/10/2017
      - correction d'un bug dans \loi_ifcs

v1.51 24/10/2017
      - correction d'un bug dans \loi_ifcs
